Timed Automata Semantics for Visual e-Contracts

C-O Diagrams have been introduced as a means to have a more visual representation of electronic contracts, where it is possible to represent the obligations, permissions and prohibitions of the different signatories, as well as what are the penalties in case of not fulfillment of their obligations and prohibitions. In such diagrams we are also able to represent absolute and relative timing constraints. In this paper we present a formal semantics for C-O Diagrams based on timed automata extended with an ordering of states and edges in order to represent different deontic modalities.

==> eptcsdata.tex <==
\providecommand{\firstpage}{7}
\providecommand{\publicationstatus}{E. Pimentel, V. Valero (Eds.): Workshop on Formal Languages\\
and Analysis of Contract-Oriented Software 2011 (FLACOS'11)\\
EPTCS 68, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.68.3}{10.4204/EPTCS.68.3}}

